Can NetGAN be improved on short random walks?

Graphs are useful structures that can model several important real-world problems. Recently, learning graphs have drawn considerable attention, leading to the proposal of new methods for learning these data structures. One of these studies produced NetGAN, a new approach for generating graphs via random walks. Although NetGAN has shown promising results in terms of accuracy in the tasks of generating graphs and link prediction, the choice of vertices from which it starts random walks can lead to inconsistent and highly variable results, especially when the length of walks is short. As an alternative to random starting, this study aims to establish a new method for initializing random walks from a set of dense vertices. We purpose estimating the importance of a node based on the inverse of its influence over the whole vertices of its neighborhood through random walks of different sizes. The proposed method manages to achieve significantly better accuracy, less variance and lesser outliers.

==> related_work.tex <==
\section{Related work}
Several approaches have been considered in Graph Neural Networks Methods and Applications. The concept of neural network of graphs (GNN) was first proposed in \cite{Scarselli:2009:GNN:1657477.1657482}. The work \cite{Scarselli:2009:GNN:1657477.1657482} extended the existing neural networks for the processing of the data represented in the graph domains. Although the experimental results have shown that GNN is a powerful architecture for structural data modeling, there were some limitations, such as: the inefficiency in updating the hidden states of the nodes in an iterative way for the fixed point, use of the same parameters in the iteration, not achieving effectively model some informational features at the edges and it is not appropriate to use the fixed points if we focus on the representation of nodes instead of graphs.

New approaches focuses on variants operating on different graph types. These variants extend the representation capability of the original model like Directed Graphs in ADGPM \cite{DBLP:journals/corr/abs-1805-11724}, Heterogeneous Graphs in GraphInception \cite{Zhang:2018:DCC:3178876.3186106}, Graphs with Edge Information in G2S \cite{beck-etal-2018-graph} and r-GCN \cite{Schlichtkrull2018ModelingRD}.
Others researches focuses in new propagations types approaches. Four main propagations types approaches were proposed. 
1. Convolution: the authors \cite{ae482107de73461787258f805cf8f4ed} proposed the spectral network, \cite{NIPS2016_6212} proposed the diffusion-convolutional neural networks (DCNNs), \cite{NIPS2017_6703} proposed the GraphSAGE, a general inductive framework that uses an LSTM-based aggregator which has a larger expressive capability.  
2. Gate: the authors \cite{Li2016GatedGS} proposed the gated graph neural network (GGNN) which uses the Gate Recurrent Units (GRU) in the propagation step, unrolls the recurrence for a ﬁxed number of steps T and uses backpropagation through time in order to compute gradients. \cite{tai-etal-2015-improved} proposed two extensions to the basic LSTM architecture: the Child-Sum Tree-LSTM and the N-ary TreeLSTM.  
3. Attention: The attention mechanism has been successfully used in many sequence-based tasks such as machine translation \cite{Bahdanau2015NeuralMT} \cite{gehring-etal-2017-convolutional} \cite{NIPS2017_7181} and machine reading \cite{cheng-etal-2016-long}. The authors \cite{velickovic2018graph} proposed a graph attention network (GAT) which incorporates the attention mechanism into the propagation step.
4. Skip connection: The residual network was propose in \cite{7780459}. The authors \cite{pmlr-v80-xu18c} proposed the Jump Knowledge Network which could learn adaptive, structure aware representations. It uses three approaches of concatenation, max-pooling and LSTM-attention in the experiments to aggregate information.

Different variants of graph neural networks were proposed using advanced training methods, which improve the training efﬁciency. GraphSAGE \cite{NIPS2017_6703} is a comprehensive improvement of original GCN. FastGCN \cite{chen2018fastgcn} further improves the sampling algorithm. The authors \cite{DBLP:journals/corr/abs-1809-05343} introduces a parameterized and trainable sampler to perform layerwise sampling conditioned on the former layer. In \cite{pmlr-v80-chen18p} the authors proposed a control-variate based stochastic approximation algorithms for GCN by utilizing the historical activations of nodes as a control variate.

Apart from different variants of graph neural networks, several general frameworks are proposed aiming to integrate different models into one single framework. The authors  \cite{DBLP:journals/corr/GilmerSRVD17} proposed a general framework for supervised learning on graphs called Message Passing Neural Networks (MPNNs). In \cite{DBLP:journals/corr/abs-1711-07971} was propose the Non-local Neural Networks (NLNN) for capturing long-range dependencies with deep neural networks. The authors \cite{DBLP:journals/corr/abs-1806-01261} proposed the Graph Network (GN) framework which generalizes and extends various graph neural network, MPNN and NLNN approaches \cite{Scarselli:2009:GNN:1657477.1657482} \cite{DBLP:journals/corr/GilmerSRVD17} \cite{DBLP:journals/corr/abs-1711-07971}.

Deep learning methods for graph data have mostly been studied in the context of node embeddings \cite{DBLP:journals/corr/PerozziAS14} \cite{DBLP:journals/corr/GroverL16} \cite{Kipf2016VariationalGA}. The recently proposed GraphGAN \cite{DBLP:journals/corr/abs-1711-08267} is another instance of such prescribed edge-level probabilistic models, where f is optimized using the GAN objective instead of the traditional cross-entropy. The authors \cite{DBLP:journals/corr/LiuCCOYS17} propose a GAN architecture for learning topological features of subgraphs. Tavakoli et al. \cite{Tavakoli2017} apply GANs to graph data by trying to directly generate adjacency matrices.

Most approaches focus on generating discrete sequences such as text, with some of them using reinforcement learning techniques to enable backpropagation through sampling discrete random variables \cite{DBLP:journals/corr/YuZWY16} \cite{articlekusner} \cite{DBLP:journals/corr/LiMSRJ17} \cite{DBLP:journals/corr/LiangHZGX17}. Other approaches modify the GAN objective to tackle the same challenge \cite{DBLP:journals/corr/CheLZHLSB17} \cite{devon2018boundary}.
